Evaluation Metrics for Measuring Bias in Search Engine Results

Search engines decide what we see for a given search query. Since many people are exposed to information through search engines, it is fair to expect that search engines are neutral. However, search engine results do not necessarily cover all the viewpoints of a search query topic, and they can be biased towards a specific view since search engine results are returned based on relevance, which is calculated using many features and sophisticated algorithms where search neutrality is not necessarily the focal point. Therefore, it is important to evaluate the search engine results with respect to bias. In this work we propose novel web search bias evaluation measures which take into account the rank and relevance. We also propose a framework to evaluate web search bias using the proposed measures and test our framework on two popular search engines based on 57 controversial query topics such as abortion, medical marijuana, and gay marriage. We measure the stance bias (in support or against), as well as the ideological bias (conservative or liberal). We observe that the stance does not necessarily correlate with the ideological leaning, e.g. a positive stance on abortion indicates a liberal leaning but a positive stance on Cuba embargo indicates a conservative leaning. Our experiments show that neither of the search engines suffers from stance bias. However, both search engines suffer from ideological bias, both favouring one ideological leaning to the other, which is more significant from the perspective of polarisation in our society.

==> notation.tex <==
%Article Title: Measuring Search Engines' Political Bias in Controversial Topics via Stance Bias
%Journal Name: Information Retrieval Journal
%Authors: Gizem Gezici, Aldo Lipani, Yucel Saygin, and Emine Yilmaz
%Corresponding Author Information: Gizem Gezici, Sabanci University, gizemgezici@sabanciuniv.edu


Follows a set of symbols, functions, and labels used in this paper:
%\vspace{1.5em}

\begin{comment}
\begin{supertabular}{ l l }
\hline
\hline
{Symbols}\\
\hline
\hline
$\sS$   & set of search engines. \\
$s$     & a search engine $s \in \sS$. \\
$\sQ$   & set of queries. \\
$q$     & a query $q \in \sQ$. \\
%$d$     & a document. \\
$r$     & a SERP (a retrieved document). \\%(list of documents).
$r_i$   & the document in $r$ retrieved at rank $i$.\\
$|r|$   & size of $r = [r_1, r_2, \dots, r_{|r|}]$.\\
$n$     & number of documents considered in $r$ by $f$ (cut-off).\\
$G$     & a set of groups $g_i$ ($g_1 \cup g_2 \cup \dots \cup g_n = G$). \\
$g_i$   & a group $g_i \in G$. \\ \hline
%\hline
\hline
{Functions}\\
\hline
\hline
$s(q)$                  & returns $r$ given a query ($q$). \\ 
$j(r_i)$                & returns the label associated to $r_i$.\\
$j(q)$                  & returns the label associated to $q$.\\
$f(r)$                  & an evaluation measure for SERPs.\\
$f_g(r)$                & like $f$ but for $g$.\\
%$f_{-}(r)$             & like $f$ but for the against label.\\
$[\text{Condition}]$    & returns 1 if the condition is true and 0 otherwise.\\
\hline
\hline
{Labels}\\
\hline
\hline
$g_1$  & protected group. \\
$g_2$  & unprotected group. \\ \hline
$\lps$ & pro stance. \\
$\lns$ & neutral stance. \\
$\las$ & against stance. \\ 
$\lnr$ & not-relevant stance. \\ \hline
$\lcp$ & conservative political perspective.
\\
%$\lnp$ & neutral political perspective. \\
$\llp$ & liberal political perspective. \\
$\lbp$ & both or neither political perspectives. \\
%$+$ & label  .\\
%$-$ & against label.\\
\hline
\hline
\end{supertabular}
\end{comment}
%\end{center}
%\end{table}

==> our_method.tex <==
%!TEX root = main.tex

In this section, we present the core components of our unsupervised key-phrase extraction pipeline. Our pipeline is composed of three main parts. First, we extract informative noun-phrases as candidates from a given document. Then, these candidates and the current document are represented in a high dimensional vector space using sBERT. Lastly, we rank the candidate phrases by using the cosine similarity scores. A simple flowchart explaining this process can be seen in \ref{fig:sBERT_figure}.

%Commented code
\begin{figure}[!h]
\vspace{-1.6em}
\centering
\begin{tikzpicture} [
block/.style={rectangle, draw=black!60, very thick, minimum width=30mm,  minimum height=8mm, node distance=0.45cm},
] 

\node[] (input) {{sent}};

\node[block] (np_chunker) [below=of input] {Noun-Phrase Chunker};

\node[] (output_1) [below=of np_chunker] {list of ${NP}$};

\node[block] (sbert) [below=of output_1] {sBERT};

\node[] (output_2) [below=of sbert] {list of candidate embeddings};

\node[block] (rank_cand) [below=of output_2] {Ranking Candidates};

\node[] (output_3) [below=of rank_cand] {informativeness of candidates};

\draw[->] (input.south) -- (np_chunker.north);
\draw[->] (np_chunker.south) -- (output_1.north);
\draw[->] (output_1.south) -- (sbert.north);
\draw[->] (sbert.south) -- (output_2.north);
\draw[->] (output_2.south) -- (rank_cand.north);
\draw[->] (rank_cand.south) --(output_3.north);

\end{tikzpicture}
\vspace{-1em}
\caption{\label{fig:sBERT_figure}sBert-Rank Pipeline}
\vspace{-1.2em}
\end{figure}


\subsection{Noun-Phrase Chunker}
\label{sec:nounphrase}
Key-phrases are the most informative keywords or 
multiple words for the document at hand. They are mostly nouns as well as noun or adjective phrases. Hence, in this work, we aim to catch noun-phrases including adjective phrases within a given document.

%
In order to detect noun-phrases, a widely-used stable dependency parser of Stanza~\cite{qi2020stanza} proposed by the Stanford NLP Group is used. The current document is first split into , and these sentences are given to the Stanza as inputs to generate its dependency tree for the sentences in the document. This allows us to generate dependency trees both for long and short documents. Since dependency trees contain valuable word- information, after creating the dependency tree for a given document, its noun-phrases are extracted with a rule-based approach which leverages the dependency tree information.

%
To exploit dependency tree information, we propose a one general rule where we consider a noun-phrase (\emph{NP}) as a recurrence relation. The general rule is defined as follows:

%
\begin{linenomath*}
\vspace{-0.4em}
\begin{equation}\label{eq:delta_bias}
    NP = (NOUN, ADJ)(NP)
\end{equation}
\vspace{-0.4em}
\end{linenomath*}
%

In the given rule, $NP$ initially starts with a noun or adjective, then it is followed by a noun-phrase itself. Furthermore, if we consider a given ${NP}_i$, which is comprised of $n$ tokens in total we define each of these tokens as $t_j$, where $j = 1, 2, 3, ... n$. Note that ${NP}_i$ is defined as a list of $n$ tokens with the order of ${t_1, t_2, t_3, ..., t_n}$. Then, our rule requires that the head of each $t_i$, $ 1 \leq i \leq n$, extracted from the dependency tree, which is denoted as $h(t_i)$, should be $t_n$. That is, all of the tokens within the noun-phrase should be modified by the last token. 
%
This condition helps us to filter the noun-phrases in such a way that each candidate is a complete phrase by itself. Thus, as mentioned in Section~\ref{sec:introduction} differently from~\cite{bennani2018simple} which uses only POSTag information in the candidate generation step, we obtain a more distilled set of candidate phrases using dependency tree information. In this way, the distilled set generally provides more informative candidates which are smaller in size than the ones generated by~\cite{bennani2018simple} which could provide a more effective as well an efficient processing of the documents in a given dataset. Note that for each document, only distinct noun-phrases are taken. Apart from these, since stanza is available for more than 70 languages~\footnote{\url{https://stanfordnlp.github.io/stanza/}}, the first step of our pipeline can easily be extended to extract key-phrases in other languages.

\begin{table*}[!t]
    \vspace{-0.8em}
    \centering
    \caption{Performance of sBERT-Rank on INSPEC, DUC2001, NUS and SemEval2017 Datasets}
    \vspace{-1em}
    \setlength{\tabcolsep}{3.0pt}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc}
        \hline\hline
        & & &  INSPEC & & &  DUC2001 & & &  NUS & & & SemEval2017\\
        \hline
        N & Model & R & P & F1 & R & P & F1 & R & P & F1 & R & P & F1 \\
        \hline\hline 
        \multirow{6}{*}{5} 
        & MultipartiteRank &
        0.21 & 0.28 & 0.24 & 
        0.18 & 0.15 & 0.16 &
        0.10 & 0.19 & 0.13 &
        0.11 & 0.34 & 0.16\\
        & SingleRank &
        0.2 & 0.26 & 0.23 &
        0.11 & 0.10 & 0.10 &
        0.02 & 0.04 & 0.03 &
        0.11 & 0.34 & 0.17 \\
        & TopicRank &
        0.21 & 0.28 & 0.24 &
        0.16 & 0.14 & 0.15 &
        0.09 & 0.17 & 0.12 & 
        0.10 & 0.34 & 0.16 \\
        & EmbedRank &
        0.25& 0.41& 0.31&
        0.22 & 0.34 & 0.27&
        0.02 & 0.05 & 0.03&
        0.13 & 0.45 & 0.20 \\
        & SIFRank &
        0.21 & \textbf{0.43} & \textbf{0.29} &
        \textbf{0.25} & \textbf{0.40} & \textbf{0.31} &
        0.03 & 0.04 & 0.03 & 
        \textbf{0.15} & \textbf{0.50} & \textbf{0.23}\\
        & sBERT-Rank &
        \textbf{0.28} & 0.29 & \textbf{0.29} &
        0.24 & 0.22 & 0.23 &
        \textbf{0.14} & \textbf{0.18} & \textbf{0.15} &
        0.13 & 0.32 & 0.19 \\
        
        \hline
        \multirow{6}{*}{10} 
        & MultipartiteRank &
        0.33 & 0.24 & 0.28 &
        0.26 & 0.12 & 0.17 &
        0.17 & \textbf{0.16} & \textbf{0.17} & 
        0.18 & 0.28 & 0.22\\
        & SingleRank &
        0.37 & 0.26 & 0.30 &
        0.22 & 0.11 & 0.14 &
        0.05 & 0.05 & 0.05 & 
        0.21 & 0.33 & 0.26\\
        & TopicRank &
        0.31 & 0.23 & 0.27 &
        0.25 & 0.11 & 0.15 &
        0.14 & 0.14 & 0.14 & 
        0.17 & 0.27 & 0.21 \\
        & EmbedRank &
        0.40 & 0.35  & 0.37 &
        0.35 &  0.28 & 0.28 &
        0.05 & 0.06 & 0.05 & 
        0.23 & 0.40 & 0.30 \\
        & SIFRank &
        0.39 & \textbf{0.39} & \textbf{0.39} &
        0.37 & \textbf{0.30} & \textbf{0.33} &
        0.04 & 0.04 & 0.04 & 
        \textbf{0.26} & \textbf{0.45} & \textbf{0.33} \\
        & sBERT-Rank &
        \textbf{0.43} & 0.24 & 0.31 &
        \textbf{0.39} & 0.19 & 0.25 &
        \textbf{0.22} & 0.14 & \textbf{0.17} & 
        0.24 & 0.29 & 0.26\\
        
        \hline
        \multirow{6}{*}{15} 
        & MultipartiteRank &
        0.43 & 0.22 & 0.29&
        0.33 & 0.11 & 0.16 &
        0.22 & \textbf{0.14} & \textbf{0.17} & 
        0.24  & 0.26  & 0.25 \\
        & SingleRank &
        0.47 & 0.24 & 0.32 &
        0.29 & 0.09 & 0.15 &
        0.08 & 0.05 & 0.06 &
        0.29 & 0.30 & 0.29 \\
        & TopicRank &
        0.38 & 0.21 & 0.27 &
        0.31 & 0.09 & 0.14 &
        0.17 & 0.11 & 0.13 & 
        0.22 & 0.23 & 0.22 \\
        & EmbedRank &
        0.49 & 0.31 & 0.38 &
        0.44 & 0.24 &  0.31 & 
        0.07 & 0.05 & 0.06 & 
        0.32 & 0.37 & 0.34 \\
        & SIFRank &
        0.48 & \textbf{0.33} & \textbf{0.39} &
        0.45 & \textbf{0.25} & \textbf{0.32} &
        0.06 & 0.04 & 0.05 & 
        \textbf{0.35} & \textbf{0.41} & \textbf{0.38} \\
        & sBERT-Rank &
        \textbf{0.52} & 0.21 & 0.30 &
        \textbf{0.50} & 0.16 & 0.24 &
        \textbf{0.28} & 0.12 & \textbf{0.17} & 
        0.32 & 0.26 & 0.29 \\
        
        \hline\hline
    \end{tabular}
    \label{tab:key-phrase}
    \vspace{-1em}
\end{table*}

\subsection{sBERT}
After obtaining the unique noun-phrases which are the candidates for each document, it is necessary to assess the informativeness level of each unique noun-phrase for the document to which it belongs. For this, candidate phrases and the document itself are represented in a high-dimensional vector space by using sBERT embeddings. sBERT modifies the pre-trained BERT network by using siamese networks to derive semantically meaningful sentences. Yet, in the scope of this work, we use sBERT not only for sentences, but for computing semantic textual similarity~\footnote{\url{https://www.sbert.net/}}. sBERT specifically provides a pre-trained model for English as well as a multilingual model for other languages. Thus, in addition to the first step of sBERT-Rank, the second step can easily be extended to other languages as well by using the multilingual model of sBERT.


%in order to assess the informativeness level of each unique noun-phrase for the document to which it belongs to, 

%assess how representative a noun-phrase of a document, we map the candidate and the document itself to a high dimensional vector space with the help of sBERT. sBERT is available as both English specific and multilingual pretrained models. Both aforementioned models have been employed in this work individually. An ensemble method might also be used in the future studies to achieve higher scores.

\subsection{Ranking Candidates}
In the last step of our pipeline, for ranking the candidate phrases that are represented in a high-dimensional space, two cosine similarity scores are computed. First, the cosine similarity scores between each sentence in the current document and the document itself are computed. Then, the cosine similarity scores between each candidate phrase and the sentence from which the phrase is extracted are also computed. In this way, the informativeness level of each candidate phrase is calculated by multiplying the computed cosine similarity scores. After that, the candidate phrases are ranked with respect to their informativeness level scores in ascending order. 

%
Let's assume that a given document ${doc}_i$ contains $n$ sentences. As the first step, ${doc}_i$ is splitted into its sentences of ${sent}_j$ for $j = 1, 2, 3, ... n$. Then, each sentence ${sent}_j$ is given to the Stanza and based on the dependency tree information and the rule-based approach let's assume that in total $m$ candidate phrases are extracted from ${sent}_j$. In this case, for each candidate phrase ${cand}_k$ where $k = 1, 2, 3, ... m$, the informativeness level of ${inf}_{{cand}_k}$ is computed as follows:


\begin{equation}
    \label{eq:similarity}
    {inf}_{{cand}_k} = cos ({cand}_k, {sent}_j) * cos ({sent}_j, {doc}_i)
    \vspace{1em}
\end{equation}

Note that $cos(a,b)$ computes the cosine similarity score between the textual contents of $a$ and $b$. In Eq.~\eqref{eq:similarity} the first component is the cosine similarity score computed between the candidate phrase and the sentence; while, the second component denotes the similarity score between the sentence and the whole document. After computing the score of ${inf}_{{cand}_k}$ for all $m$ extracted candidate phrases in ${sent}_j$, we fulfill the same computation for all the candidate phrases of $n$ sentences. Then, for each document ${doc}_i$, all of these scores are aggregated into a list which is sorted with respect to the computed informativeness level scores -- the candidate phrases with higher scores are expected to be more informative about ${doc}_i$.
 

%Let's assume that using the noun-phrase rules, we extract $n$ candidate phrases. Then, in the second step we represent these phrases in a high-dimensional embedding space using sBERT. Let $\set{P}$ be a set of the high-dimensional representations of these candidate phrases. and when we compute a score for $p_i \in \set{P}$ where $i = 1, 2, 3, ... n$, 


%let's say we extract $n$ candidate phrases using the Stanza dependency parser in the first step of the pipeline. Then, ewch


%The equation for computing the score of a given candidate phrase can be seen in Eq.~\eqref{eq:similarity}.


%the informativeness of each candidate phrase is calculated using the both of these similarity scores. as the multiplication of both cosine similarity scores where a high similarity with a sentence means little if the sentence is not informative of the document at all. Then, of course, the candidates are ranked with respect to their scores in ascending order. The equation to calculate the ranking score of a candidate can be seen in Equation \eqref{eq:similarity}.











